Daydream: Accurately Estimating the Efficacy of Optimizations for DNN Training

Modern deep neural network (DNN) training jobs use complex and heterogeneous software/hardware stacks. The efficacy of software-level optimizations can vary significantly when used in different deployment configurations. It is onerous and error-prone for ML practitioners and system developers to implement each optimization separately, and determine which ones will improve performance in their own configurations. Unfortunately, existing profiling tools do not aim to answer predictive questions such as "How will optimization X affect the performance of my model?". We address this critical limitation, and proposes a new profiling tool, Daydream, to help programmers efficiently explore the efficacy of DNN optimizations. Daydream models DNN execution with a fine-grained dependency graph based on low-level traces collected by CUPTI, and predicts runtime by simulating execution based on the dependency graph. Daydream maps the low-level traces using DNN domain-specific knowledge, and introduces a set of graph-transformation primitives that can easily model a wide variety of optimizations. We show that Daydream is able to model most mainstream DNN optimization techniques, and accurately predict the efficacy of optimizations that will result in significant performance improvements.

==> Makefile <==
PAPER = paper
TEX = $(wildcard *.tex sections/*.tex figNodes/*.tex)
BIB = paper.bib
FIGS = $(wildcard plots/*.pdf plots/*.png)

.PHONY: all clean

$(PAPER).pdf: $(TEX)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi *.gz \
	$(PAPER).pdf


==> key_idea.tex <==
\vspace{-2mm}
\section{Key Ideas} \label{sec:idea}
\vspace{-1mm}

In this section we highlight the key ideas and observations behind the \system{} design.

\textbf{Constructing kernel-granularity dependency graph.} The neural network topology is a natural graph structure in which nodes are DNN operators or layers. Most mainstream DNN frameworks~\cite{mxnet,pytorch}
provide built-in tools to record the layer-level runtime profile.
The layer-level abstraction is intuitive for programmers to understand the "where time goes" question, but hides important information about the parallel execution of the CPU functions, GPU kernels, and memory transfers.
This information is crucial for accurate performance predictions. For example, optimizations that reduce numerical precision will change the duration of GPU kernels while the CPU runtime remains unchanged, and optimizations like vDNN~\cite{vdnn} will inject CUDA memory copies, without changing the duration of GPU kernels.
%With a dependency graph in the layer-level abstraction, we need to accurately predict how the duration of each layer changes when applying these optimizations, which is very hard due to the missing low-level details.
It is extremely hard to predict how duration of each layer changes when applying these optimizations if lacking low-level details about CPU and GPU runtime.
%Figure~\ref{fig:details_of_a_layer} shows one representative example of a potential runtime complexity within one layer, and how the performance bottleneck could shift between CPU and GPU. 
%It is not trivial to estimate how its runtime scales with the scaling of internal GPU kernels' duration.
%Hence, using only layer-level abstraction, it would be difficult to evaluate the efficacy of many optimizations (e.g., mixed precision~\cite{micikevicius2017mixed}, FusedAdam~\cite{apex_opt}, restructuring batchnorm~\cite{jung2018restructuring}). 
To accommodate optimizations that target fine granularity tasks (such as GPU kernels), our proposed system, \system{} chooses to model the training workloads using a kernel-level dependency graph (i.e., each GPU kernel has one corresponding \task{} in the graph), incorporating detailed traces of CPU, GPU and communication runtime.

\begin{figure}
    \includegraphics[width=\columnwidth]{figures/nvprof_resnet50.pdf}
    \caption{NVProf timeline example of training ResNet-50.}
    \label{fig:nvprof_screenshot}
    \vspace{-4mm}
\end{figure}

%Figure~\ref{fig:mxprofile} shows a fragment of the profile generated by MXNet (opened with \url{chrome://tracing}). One box in this profile represents the forward phase of one layer. It shows how much time does each layer spend in a succinct way, but does not expose details inside the runtime of a layer (e.g., how much time is spent on CPU or GPU).

% we probably need to cite some article where people use such a trivial strategy to predict performance with TensorCores
%The layer-level granularity could be incompetent to model optimizations that %improve hardware computation.
%One of such examples is the mixed precision~\cite{das2018mixed} technique.
%If we estimate the overall performance by scaling each layer by 2x, we are very likely to predict the overall speedup to be close to 2x (and higher when considering Tensor Cores).
%However, as we show later in Section~\ref{sec:eval:amp}, the speedup of mixed precision is mostly much lower than 2x.
%Such prediction error is due to lack of low-level runtime information.
%The runtime scale of any given layer depends on the concurrency between the CPU and GPU runtime, and the types of GPU kernels (compute-bound or memory-bound).
%Hence, to accurately estimate such optimizations, it is necessary to model them in the kernel-level abstraction.

%DNN training is an iterative algorithm that each iteration performs the same forward and backward computation. Predicting performance should be based on profiles from at least one iterations. A kernel-level \task{} could be less than twenty microseconds. Nevertheless, one DNN training iteration typically takes a few hundreds milliseconds. This suggests that the number of \task{}s in a graph is expected to be at least hundreds or even thousands. Manually adding dependencies for all \task{}s will be challenging as the dependency graph topology could be very complicated.
%When predicting performance of optimizations like kernel fusion, or distributed training from the single-worker profile, we need to add \task{}s to the dependency graph for further analysis.
With a large number of kernel-level \task{}s that are spread across several threads and CUDA streams, the complexity of constructing the dependency graph comes mainly from identifying the inter-thread dependencies~\cite{von2008modeling}.
Existing tools do not provide such dependency tracking.
We make the following key observations about the DNN training workloads to overcome this general challenge of dependency tracking in concurrent systems.
First, for the implementations in the mainstream frameworks~\cite{mxnet,pytorch}, once a mini-batch has been prepared by data loading threads, only one or two CPU threads are involved in the control flow of computation.\footnote{Our approach can be generalized to frameworks that use more concurrent CPU threads.}
Second, there is a very limited number of concurrent GPU kernels. Such serialization of GPU kernels is due to two main reasons: (i) GPU kernels in the modern cuDNN library achieve high GPU core utilization; (ii) ML frameworks usually invoke only one CUDA stream.
Figure~\ref{fig:nvprof_screenshot} shows the NVProf profiles of one training iteration of ResNet-50.
There are two CPU threads involved, but no CPU \task{}s run concurrently. The high serialization of low-level traces is not a unique phenomenon for just convolutional networks. We observe a similar phenomenon in most DNN training workloads.

Based on these insights, \system{} constructs the kernel-level dependency graph in three major steps. First, \system{} uses CUPTI to extract traces of all GPU kernels, CUDA memory copies, and CUDA APIs. Second, \system{} captures the dependencies between CPU and GPU \task{}s, caused by CUDA synchronizations and GPU kernel launches. Third, when predicting performance for distributed training, \system{} adds communication \task{}s to the dependency graph.

%There are three main reasons that cause the \task{}s to be highly serialized: (i) the implementation of mainstream DNN frameworks rarely invoke sub-processes; (ii) the GPU kernels in modern cuDNN library achieve high GPU core utilization; (iii) some mainstream frameworks invoke only one or very few GPU streams. Based on these observations, the massive amount of low-level \task{}s belong to a very limited number of serialized threads (one CPU thread, one GPU thread and one or two communication threads), and we only need to determine the inter-thread dependencies.

\textbf{Synchronization-free \task{}-to-layer mapping.} In distributed training, mainstream frameworks implement the wait-free backpropagation strategy~\cite{zhang2017poseidon} to overlap communication with computation.
This strategy immediately transfers gradients once they are computed by corresponding backward layers. 
To properly add dependencies related to communication \task{}s, we need the \task{}-to-layer mapping to know when the computation of each layer ends.
Meanwhile, accurately modeling DNN optimizations by changing the graph potentially requires this \task{}-to-layer mapping to determine which \task{}s are involved and how to change them.

Unfortunately, vendor-provided tools like CUPTI do not have the required knowledge about these applications and building such a mapping requires extra DNN framework instrumentation.
A na\"ive approach to achieve this mapping is to compare the start and stop timestamps of GPU kernels and DNN layers.
This requires additional CUDA synchronization calls for each layer since GPU kernels are launched asynchronously. However, such synchronizations might significantly alter the execution runtime by adding additional dependencies from GPU to CPU \task{}s. Hence, we design a synchronization-free procedure to achieve this mapping by instrumenting timestamps for each layer in the frameworks, and utilizing the correlations between CPU and GPU \task{}s. 

\textbf{Representing complex optimizations with simple graph-transformation primitives.} As shown in Table~\ref{table:approches}, DNN optimizations target a wide range of performance bottlenecks with various approaches.
Unlike prior dependency graph analysis in non-ML contexts~\cite{curtsinger2015c,ousterhout2015making,ousterhout2017monotasks}, where users can model most what-if questions by simply shrinking and scaling \task{} runtime, accurately modeling DNN optimizations with the low-level dependency graph might require complicated changes to the dependency graph.
Manually changing the kernel-level graph to model optimizations could be both complicated and error-prone, and the programmers might simply opt to rather directly implement the optimizations.

To address this problem, we propose a small set of graph-transformation primitives, so that popular optimization techniques can be effectively represented as a combination of these primitives.
These primitives include (i) \task{} insertion/removal, (ii) \task selection and update, and (iii) changing the policy for scheduling \task{}s.
The proposed primitives are simple yet powerful enough to represent many different optimizations as we will show in Section~\ref{sec:reduce}. They play a key role in realizing our goal of efficiently exploring what-if questions.

In summary, Daydream introduces the abstraction of a kernel-granularity dependency graph that contains mappings back to DNN specific abstractions (layers).
It tracks dependencies by collecting profiling data as well as instrumenting DNN frameworks.  
Daydream also provides primitives to mutate the dependency graph in the form of simple graph transformations.  
Altogether this enables programmers to both (i) model a diverse set of popular optimizations spanning kernel- and layer-level enhancements by using simple graph-transformation primitives, and (ii) estimate the efficacy of optimizations by simulating execution time based on optimization-induced graph mutations.

%The design of \system{} considers not only how to construct the graph (so that we can accurately simulate the execution), but also how to properly modify the graph according to common optimizations for DNN training. Describing these optimizations often requires concepts across different levels of abstractions. One of the examples is the FusedAdam optimizer provided by NVidia's Apex package. This optimizer fuses all kernels in the Adam optimizer into one single kernel. To properly change the graph, we need to know which \task{}s belong to the weight update phase. It is very onerous to manually add/delete node by node and edge by edge in a kernel-level dependency graph. To enable easy and accurate graph modification based on optimizations require: (1) mapping \task{}s to DNN layers; (2) introducing a set of graph-changing rules that are easy to use.

==> sections/introduction_.tex <==
\section{Introduction}

%A modern NVidia V100 GPU contains 5120 cores, 10 times compared to the GTX 580 GPU that was used to train AlexNet~\cite{krizhevsky2012imagenet} in 2012. Beyond GPUs, architects also proposed other new accelerators (e.g., TPU~\cite{tpu}, Microsoft Catapult~\cite{putnam2014reconfigurable}, Amazon Inferentia~\cite{inferentia}) to improve the DNN computation performance. Meanwhile, system researchers and developers built software stacks for ML programmers to efficiently harness the power of the underlying hardware. DNN frameworks (e.g., Theano~\cite{bergstra2010theano}, MXNet~\cite{mxnet}, TensorFlow~\cite{tf}, PyTorch~\cite{pytorch}) provide portable programming APIs for ML programmers to design DNN algorithms, and employ compilers (e.g., XLA~\cite{xla}, TensorRT~\cite{tensorrt} and kernel libraries (e.g., cuDNN~\cite{chetlur2014cudnn}, MKL~\cite{wang2014intel}) to optimize the DNN computation. Despite this advancement in hardware/software support in DNN computation, ML researchers come up with new innovations at a breakneck pace~\cite{devlin2018bert}~\cite{he2017mask}~\cite{resnet}~\cite{vaswani2017attention}. Hence, the demand for more computing keeps growing~\cite{schwartz2019green}.

%Despite that the hardware/software support is always advancing, the demand for more computation power never declined. ML researchers keep develop new DNN models with better accuracy that require more computation power to train. In 2012, training AlexNet on two GTX 580 GPUs takes five to six days~\cite{krizhevsky2012imagenet}. In 2014, training the GoogLeNet with high-end GPUs at that time, also took close to a week~\cite{szegedy2015going}. In 2018, training BERT, which is the state-of-the-art model for language modeling, still takes four days to train on 16 TPUs~\cite{devlin2018bert}.

Recent years have witnessed the co-evolution of deep neural network (DNN) algorithms and the underlying hardware and software design.  
Machine learning (ML) researchers come up with new innovations at a rapid pace~\cite{devlin2018bert}~\cite{he2017mask}~\cite{resnet}~\cite{vaswani2017attention}. 
%gena: we need to elaborate on these innovations at least briefly, otherwise it is too high-level
Motivated by these workloads, hardware architects have designed a range of accelerators to efficiently execute them: from GPUs, to ASICs and FPGAs (e.g., TPU~\cite{tpu}, Microsoft Catapult~\cite{putnam2014reconfigurable}, Amazon Inferentia~\cite{inferentia}).
%gena: some of your sentences are not technically correct, like GPUs were not designed specifically for any of these workloads, just optimized a bit
% In general, I would reorganize the first two sentences to reflect a slighly different argument:
% 1. ML researchers came up with many important models ... that have a huge increase in compute depand (cite open-ai and other relevant examples on huge compute demand). 2. Computer architects respond to that with different hardware accelerators (as general-purpose is not efficient enough).
%3. But these hardware accelerators won't provide much without proper software optimization across the full systems stack. 
% As the results, systems researchers ...
To meet the demand for fast DNN computation, system researchers have been proposing a variety of performance optimizations, targeting different bottlenecks across the system stack \--- for example, improving memory utilization, better parallelization, and improving communication.
%gena: citations are missing 
%One way commonly used to reduce DNN training time is leveraging multiple hardware accelerators via data parallelism~\cite{bottou2010large}. 
Moreover, researchers have also developed workload-centric optimizations. 
%gena: I'm not sure I agree with your definition of workload-centric. Some people might thing about models there, rather than distributed training
% you need to be more precise.
For example, precision reduction~\cite{das2018mixed}~\cite{gupta2015deep}~\cite{micikevicius2017mixed} aims to optimize runtime as well as memory consumption, and gradient compression~\cite{lu2018multi}~\cite{lin2017deep} aims to reduce the communication overhead in distributed training.

Despite these advances, it is common for users to ask performance questions such as:
%gena: this connection does not sound great to me. I don't see the connection between optimizations, and performance questions. You need to elaborate on it.

\textit{Why did my DNN training workload run slowly?  Will performance optimization X help me?  Is the amount of memory on my GPU limiting performance?  How much will upgrading from a 10Gbps to a 100Gbps network improve training throughput?  How will my workload scale with twice the number of GPUs?}
%gena: I like the idea on listing several example questions you want to answer, but we need a better structure.

Unfortunately, it is not easy to answer these questions today.  %gena: today sounds too colloquial. In modern systems or frameworks?
%gena: Nice list, but needs a better structure
% There are X major challenges to ...
%First, ... Second, ... Third, ...
The efficacy of many proposed performance optimizations can change significantly when applied to different ML models and deployment configurations. 
The hardware deployments that practitioners use tend to be heterogeneous; models might run on a different hardware configuration as those used by the inventors of the models.
%and the initial developers of performance optimizations. 
Differences in accelerator type, compute capabilities, available memory, networking capabilities, and software library versions can all change the major bottlenecks in the execution of these models.
%gena: you need to structure your arguments a bit better. Heterogeneity of hardware configurations, software tools, and models should be probably merge into one strong argument. Second, limitations of existing profiling tools. 
Profiling tools provided by hardware vendors (e.g., NVProf~\cite{nvprof}, Nsight~\cite{nsight}) or DNN frameworks do not offer the right abstractions to help programmers identify performance bottlenecks and they are not effective in estimating the efficacy of potential performance optimizations.
As a result, it is hard for programmers to harness profiling data to identify performance bottlenecks, and it is equally onerous for them to implement and evaluate various optimizations to identify the ones that actually work.

%gena: we already had one list of questions, now we have another one. We need to make sure those are either the same or very well connected
The central focus of this paper is to answer the following question for DNN training workloads: \textit{Given a model and a potential deployment scenario, how can we efficiently explore the efficacy of potential solutions}?
%gena: you didn't define what-if questions
Profiling to explore what-if questions requires reasoning at a level of \textit{abstraction} that is easy for analysis, and for it be \textit{accurate} (capture parallel execution, asynchrony, and interference) and \textit{complete} (CPU, GPU, Network).
%gena: your summary is okaying, but it sounds too incremental. You start with a graph dependency analysis which is a very well-known idea.
% I suggest to write by saying that we make a key observation that using dependency graph analysis in this context is simpler than general context.
Our proposed approach is based on the \emph{dependency graph analysis}, which decomposes the training workload into a group of \emph{\task{}s}, and structures these \task{}s using a dependency graph. When answering the what-if question given an optimization, we predict the runtime by modifying the graph accordingly and simulating the execution. 
%gena: I don't like the flow here, you use the term task, and then decided to define it properly. This needs serious revision.

The definition of a \emph{\task{}} in the dependency graph is the basis for further performance reasoning. DNN training workloads heavily rely on accelerators such as GPU. Various optimizations (cite a lot) focus on utilizing GPU more efficiently. To properly model the impact of these optimizations (i.e. being able to model changes of individual GPU kernels), the \task{} granularity should be fine-grained enough. This raises two challenges: (i) constructing the graph is hard, because a graph is expected to have thousands of \task{}s and no existing tool can automatically add dependencies among them; (ii) modifying the graph to properly model an optimization is hard, because a \task{} is extremely low-level.

%However, this is difficult because of three main reasons.
%First, existing profiling tools such as NVProf and Nsight provide kernel-level profiling data, but the granularity of profiling complicates reasoning about DNN-training-targeted performance bottlenecks.  On the other hand, operator-level (or layer-level) profiling in DNN frameworks simplify reasoning about bottlenecks, but profiling can be incorrect due to asynchrnous GPU kernel launches (underestimating actual execution time) or due to forced synchronous calls (which get individual kernel execution times right, but cannot capture parallel execution of CPU and GPU operations).
%Second, a complete profile ought to also capture timing information about CPU side activities such as memory allocation, tensor initialization, and kernel launches.
%Third, to reason about the efficacy of optimizations for distributed training, a complete and accurate model of interference (contention for CPU and GPU resources) between overlapping computation and communication tasks in DNN training is essential, but there is no such model available today. 

%Each of these strategies aim for specific types of performance bottlenecks. These optimization efficiency depends on the configurations of the full ML stack. Unfortunately, every layer in the full ML stack from algorithm to hardware keeps evolving, and hence the main bottlenecks in training a DNN could be quickly shifting. As a result, performance profiling becomes increasingly important for programmers to identify bottlenecks, and choose efficient optimization strategies for different DNN algorithms under different hardware/software configurations.

% For example, we observe that upgrading the version of the cuDNN library from 9.0 to 10.0 could increase the GPU compute utilization of training the Seq2Seq~\cite{seq2seq} model from less than 50\% to around 90\%, changing training Seq2Seq from a CPU-bound to a GPU-bound workload.

%\emph{Since GPU kernels are triggered asynchronously, these tools will generally add synchronizations to collect per-layer or per-operation runtime information}.

%These domain-specific tools can illustrate performance hotspots, but are less efficient in finding optimization opportunities. The main reason is because new domain-specific optimization techniques keep emerging. The efficiency of these new techniques (e.g., kernel fusion, precision reduction) often depends on specific bottlenecks that current domain-specific tools cannot reveal. For example, when a certain DNN layer takes a long time, should we try to improve its kernel implementation, reduce value precision, fuse it with another layers, or do a combination of these? It is also possible that we have already reached the theoretical best performance for this layer and the only approach to improve performance further is to use a better hardware accelerator. As a result, programmers often have to try various optimization techniques only to find out most of them are not useful.

%Profiling plays a key role in helping programmers identify major bottlenecks and efficient optimizations for specific workloads and system configurations. Programmers usually have to rely on profiling tools provided by hardware vendors (e.g., NVProf~\cite{nvprof}, Nsight~\cite{nsight}) or profiling tools built in DNN frameworks (e.g., TensorFlow~\cite{tf}, MXNet~\cite{mxnet}, PyTorch~\cite{pytorch}). These tools are able to provide necessary information for programmers to infer performance bottlenecks, but are less effective in estimating the efficacy of potential performance optimizations. As a result, programmers have to spend extra effort themselves to harness the profiling data to identify performance bottlenecks, or in implementating and evaluating various optimizations to find out the ones that actually work for them.

%With these limitations in mind, we argue that the next generation of ML profiling tools should be \emph{aware of potential optimization strategies}, thus providing programmers with useful hints about the optimization strategies that are potentially useful for their models and system configurations. The main challenge in achieving this goal, is to analyze the performance bottlenecks that can be potentially optimized by various strategies, and estimate performance gain from applying them. In this work, we argue that we need to (i) analyze performance bottlenecks with CPU and GPU runtimes considered separately, (ii) use a new synchronization-free approach to map the low-level GPU kernels to high-level DNN structures, and (iii) predict runtime performance for distributed training.

%It can provide programmers directly hints about which strategies are the most efficient, before spending the effort to implement each of them. We use the idea of simulating runtime, similar to~\cite{ousterhout2015making}, to predict the performance of distributed training using profiling data collected only from a single-GPU configuration. We will show that communication and computation is not as isolated as people usually thought. Predicting communication time accurately has to take computation into account.

To achieve our goal to answer potential what-if questions, we introduce \emph{\system{}}, a new system that addresses the two key challenges described above.
\system{} constructs the dependency graph by utilizing the fact that \task{}s are highly sequential.
The dependency graph provides a realistic model of overlapping among CPU, GPU and communication runtimes in a DNN training workload. 
It uses a new synchronization-free approach to map low-level GPU kernels onto appropriate higher-level DNN layer abstractions. 
We also introduce a new language, which contains succinct operations to the dependency graph. This allows programmers to accurately depict a performance optimization.
%gena: did you come up with a better term than language?
In our evaluation, we show that \system{} is able to accurately predict the performance of various optimizations within 20\% error.  
%gena: we need a better way to describe our results, just 20% error sounds too high, and does not reflect what you can do. What is more important
%your system accurately predict the usefulness of different optimizations in different contexts.
This allows programmers to understand which optimization strategies are potentially efficient, and to find new opportunities that current profiling tools cannot. %gena: English is still quite poor in many of the sentences here.
%effectively detect for state-of-the-art models such as Deep Speech 2~\cite{gupta2015deep} and BERT~\cite{devlin2018bert}. 
%It is also able to predict the performance of data-parallel distributed training with less than 10\% error for most DNN applications, under various network bandwidth and system configurations.

%increasing the performance by at least 15\% with less than 30 lines of code changes.

In summary, this paper makes the following contributions:

\begin{itemize}
    \item We make a key observation, that fine-grained \task{}s in one DNN training workloads are highly sequential. %gena: sequential.
    This makes constructing a dependency graph with \task{}s feasible. %gena: you need to elaborate more here, but I like this contribution.
    \item We propose \system{}, a new system that can automatically (i) collect profiling data by instrumenting DNN frameworks and using CUPTI~\cite{cupti}, (ii) construct the dependency graph based on collected data, (iii) simulate the execution based on the dependency graph to predict the performance.
    \item We design some rules to help programmers to change the graph and model the impact of potential optimizations. We show that with these rules, we can easily and accurately depict a wide range of optimizations, which goals range from improving hardware utilization to reducing communication overhead.
    %gena: "designing some rules" does not sound exciting. We need to find a better term.
    %gena: say how many optimizations and optimization types we covered.
    \item We extensively evaluate \system{}, with five different optimizations on different models and system deployments. In all of our evaluations, \system{} is able to predict the performances within 20\% error. Furthermore, using only one GPU, \system{} is able to predict distributed training runtime for most configurations within 10\% error. 
    %gena:  I don't think you focus on the right thing. You focus on the error %, while it is more important on whether people make the right decision about useful vs. non-useful optimization.
    %\item \system{} is able to produce complete and accurate performance profiles with a modest overheard;  for four DNN models it incurs a 15\% median (up to 25\% max) runtime overhead.  \system{} profiles enable us to quickly analyze the efficacy of different optimizations on four different DNN models.  We are also able to identify new opportunities for performance optimizations, overcoming CPU bottlenecks in training Deep Speech 2~\cite{gupta2015deep} and BERT~\cite{devlin2018bert}, resulting in a modest  15\% improvement in training time with less than 30 lines of code changes.  Furthermore,  using only one GPU, \system{} is able to predict distributed training runtime for most models within 10\% of the actual training time.
    %We extensively evaluate \system{}, achieving accurate prediction of distributed training for different models and system deployments, and find new opportunities to improve training performance by reducing CPU overhead for multiple models. These opportunities are not widely noticed due to lack of proper profiling tools, but are effective (15\% speedup without sacrificing training accuracy).
\end{itemize}

==> sections/motivation.tex <==

\section{Challenges} \label{sec:motiv}

%Existing profiling tools have three major limitations in identifying performance bottlenecks and estimating potential benefits of different optimization strategies. 
%These limitations motivate the design of a new profiling tool proposed in this paper.
%The DNN training performance is sensitive to not just the DNN algorithms, but also the underlying hardware/software configurations. Profiling tools are widely used by programmers to identify bottlenecks under different configurations for different DNN models. We propose a new profiling tool, called \emph{\system{}}, that is motivated by three major limitations and pitfalls of main-stream profiling tools for DNN training.

%Hardware profiling tools (e.g. NVProf~\cite{nvprof}) provide comprehensive low-level runtime details for programmers to harness. To identify the performance bottlenecks from those low-level details, programmers need experience in system, hardware, and even machine learning to know which details are crucial. Sometimes it requires further engineering effort to organize these details properly.

%Framework built-in tools often generate layer-wise execution timeline, which is more intuitive than simply revealing hardware counters. A layer-wise timeline view can help programmers see the performance hotspots, but still not fully capable to suggest efficient optimizations. For example, when a certain DNN layer takes a long time, should we try to improve its kernel implementation, reduce value precision, fuse it with another layers, or do a combination of these? It is also possible that we have already reached the theoretical best performance for this layer and the only approach to improve performance further is to use a better hardware accelerator.

%A modern DNN training system is a deep stack from high-level user programs to low-level hardware kernels. Details revealed by hardware profiling tools do not carry any knowledge about the high-level computation. 

%\textbf{1) Programmer effort.} Due to the lack of proper representation for CPU runtime in existing profiling tools, programmers have to spend extra engineering effort to be able to analyze bottlenecks on CPU. To illustrate how much engineering effort is required to understand performance bottlenecks using existing profiling tools, we show an example of profiling the training of the BERT\textsubscript{LARGE} model\footnote{See Section~\ref{sec:method} for details on BERT and BERT\textsubscript{LARGE}.}.

%Using NVProf, we find that the GPU compute utilization when training BERT\textsubscript{LARGE} is only 65\%. The weight update phase turns out to be the main bottleneck that causes GPU under-utilization. To draw this conclusion, we need to make a key observation, that the weight update phase contributes 58.5\% of the GPU idle runtime. This is hard to do using existing tools.  In addition to collecting per-kernel runtime statistics via NVProf, programmers need to (i) collect kernel-to-layer correlations by instrumenting the framework, or by utilizing the implementations of existing framework built-in tools, (ii) generate the start time and durations of time intervals when GPU is idle using per-kernel runtime statistics, and (iii) correlate these intervals to DNN layers using information collected by previous steps. To implement these steps, programmers have to write their own tools or add a substantial amount of code to the framework, which is time-consuming and error-prone. Estimating the efficacy of optimization strategies using existing profiling tools is therefore cumbersome.

%\textbf{2) Timing by adding synchronization.} To balance accuracy and completeness in profiling with ease of use, it is desirable to correlate low-level kernel details with high-level user programs. One method is to measure the compute times of each DNN layer and associate it with appropriate GPU kernel calls. However, timing layer-wise computation accurately is a non-trivial task, because GPU kernels are launched asynchronously on the CPU. Mainstream frameworks, such as MXNet~\cite{mxnet}, rely on additional synchronization calls to capture layer-wise runtime, but synchronization can lead to the improper identification of performance bottlenecks.
%For example, when measuring the per-layer runtime of training the ResNet-50 model, adding per-layer synchronization results in an execution with 62\% GPU compute utilization, leading us to believe that something other than the GPU is a major bottleneck.  But such a conclusion would be wrong, as the original run of training ResNet-50 has 95\% GPU compute utilization. Hence, we conclude that using synchronization to measure per-layer timing accurately can lead to incorrect observations.

%\textbf{3) Inability to provide performance hints.} Current profiling tools generally do not aim at providing good insights into how well an optimization technique will behave in particular contexts. 
%Framework built-in tools usually provide layer-wise computation timeline, capable of showing performance hotspots, but do not provide hints about efficacy of optimization strategies. 
%For example, when a certain DNN layer takes a long time, should we try to improve its kernel implementation, reduce value precision, fuse it with another layer, or do a combination of these? It is also possible that we have already reached the theoretical best performance for this layer, and the only approach to improve performance further is to use a better hardware accelerator. Meanwhile, strategies like precision reduction could optimize not just one but many layers, and reasoning about their efficacy requires statistics based on the complete profile of the whole training iteration. In summary, reasoning about the efficacy of these optimizations is beneficial for programmers to efficiently optimize their applications, and requires the right level of abstraction.

%Nevertheless, each optimization technique has its own trade-offs, and reasoning about optimization's performance can be helpful for programmers to choose suitable optimization strategies for their own applications. For example, in order to reduce the communication bottleneck, programmers can try to compress the gradients using deep gradient compression (DGC)~\cite{lin2017deep}, or implement priority-based parameter propagation (P3)~\cite{jayarajan2019priority} to overlap communication with computation. DGC significantly reduces the communication overhead and might be the top choice if really starving for bandwidth, but it can potentially reduce the training accuracy~\cite{lin2017deep}. P3 might bring less impressive performance improvement, but could be preferable over DGC if it provides enough improvement in communications, as P3 does not affect the training accuracy.

%, without spending extra costs to explore the strategies that might work but has little benefits. Researchers have proposed various strategies to accelerate DNN training, and each strategy has its own pros and cons.

%The major benefit of predicting distributed runtime is that it can guide developers in deciding whether it is worth to invest in better infrastructure. For example, when the performance scalability is known under different network bandwidths, developers can easily see whether it is worth purchasing high bandwidth communication (e.g., NVLink~\cite{foley2017ultra} and InfiniBand~\cite{pfister2001introduction}). Current profiling tools do not support this prediction. As we will show in Section~\ref{sec:predict}, scalability can be predicted with error generally less than 10\% at a low cost.

%\textbf{Goal.} Our goal is to build a profiling tool that can help effectively identify bottlenecks in DNN training workloads and efficiently evaluate  the efficacy of performance optimizations. We propose a new profiling tool,  \emph{\system{}}, which can provide useful hints for programmers about performance bottlenecks in their models, and accurately predict the distributed training runtime under different system configurations.

%\subsection{Limitation of Existing Profiling Tools} \label{motiv:limit}

%Profiling has in general been the key to discover performance bottlenecks and drive optimizations for DNN computations. We list three main types of such tools: the hardware profiling tools, framework built-in tools and performance oracles.

%\textbf{Hardware Profiling Tools.} Modern DNNs mostly rely on hardware accelerators like GPUs or TPUs so that the training time is tolerable. To help people understand the performance and potentially speed up the training process, the hardware and software vendors have provided various profiling tools. The most popular tools among them are the tools provided by NVidia, including nvprof, cupti and nsight. These tools expose low-level runtime details for users to harness in various scenarios. The main consideration of these tools is to expose the hardware metrics as comprehensive as possible, but due to the lack of interpretability of these details, harnessing them is not easy for most users. The profiling tools have no knowledge about the DNN computation logic, and can only deliver metrics related to the accelerators. Lots of the exposed hardware metrics, such as memory speed and function unit utilizations, can only be utilized by people with specific hardware knowledge and optimization goals. People with different goals and backgrounds will have to spend lots of time searching for the right metrics that are useful for them, and organize them to come up with optimization ideas.

%\textbf{Framework Built-in Tools.} Main-stream frameworks, such as Tensorflow or MXNet, have their own built-in profilers for users to monitor the runtime from a system's point of view. These tools usually are able to consider the DNN computation logic, and generate a higher level abstraction of the low-level runtime details provided by hardware profiling tools, by showing execution timeline composed of layer-wise computations. Comparing to the low-level tools provided by hardware vendors, these framework built-in profiling tools are able to provide a more systematic view that consider not just the accelerators, but also other parts in the system that could potentially become the bottlenecks. More importantly, these tools are able to deliver generally more intuitive views for people to identify some bottlenecks. However, the better interpretability is at the sacrifice of the comprehensiveness. These profilers usually expect their users manipulate only the user code rather than the framework code. As a result, the applicability of these tools is limited. People will have to rely on the hardware profiling tools to discover more hardcore opportunities.

%\textbf{Performance Oracles.} Recently researchers proposed several optimizations (TODO cite) to speed up training. In order to make these optimizations work under various hardware software and environments, they all have certain performance configure parameters that need to be tuned. The ranges of these parameters form a multi-dimension search space, and it relies on a search process to find the optimal configuration and deliver good enough speed-up. A performance oracle serves as a criterion of comparing any two configurations. To avoid actually executing training process for each configuration, which is usually very costly, a performance oracle usually works by collecting low-level runtime details and use them to predict the performance for each configuration. This type of profilers delivers the best interpretability that can be utilized by an auto-tuning configuring process, but worst applicability since it is designed for only for a certain optimization technique rather than a general purpose of profiling. Accurate prediction is also not required as long as the oracle is able to find the optimal or nearly optimal configuration.

%However, these tools have some common flaws which make them less efficient and convenient. For the next generation of profiling tools, we have seen several key requirements:

%\textbf{Need for Systematic Profiling.} Training a modern deep neural network requires a complex system, integrating and coordinating heterogeneous hardware components (including CPU, GPU, TPU, network, PCIe, IO devices, etc), through a complicated software stack from high-level python user code to low-level c code. Figure 1 shows how these hardware components cooperate in one training iteration. In such a complicated system, anything could contribute to bottleneck, and their bottleneck contributions could vary a lot under different software and hardware environments. The profiling tool should be able to cover the all aspects and key bottleneck potentials to avoid unexpected ones, and reveal the major bottleneck contributors under all kinds of environments.

%\textbf{Need for Fast Profiling.} Current DNN computation system is a complex software/hardware stack from the DNN algorithm to low-level hardware. Everything in this stack is moving very fast. Previous insights about bottlenecks might not be directly transferred into a new system with different DNN algorithms and hardware/software stack. As a result, in order to discover new bottlenecks, researchers have to constantly do profiling on new systems, or for their own benchmark DNNs.

%TODO: profiling within short time

%\textbf{Need for Interpretability.} Current profiling tools often provide results in one of a few forms: the values of a performance metric; a breakdown of the total runtime; or a execution timeline. These forms require certain domain expertise to read and uncover what need be done to improve performance. This is very hard to machine learning people, sometimes for system or hardware people as well. A new profiling tool should aim for reducing the human knowledge required, and provide people direct hints about speed-up potentials by predicting the performance improvement. We think showing end-to-end performance predictions is a better form to present profiling results that are more friendly to people.

%Notes: need some quantitative and concrete arguments, instead of fluffy description. Change terminologies.

%\subsection{Overview of \system{}}

%Training a modern deep neural network requires a complex system, integrating and coordinating heterogeneous hardware components (including CPU, GPU, TPU, network, PCIe, IO devices, etc), through a complicated software stack from high-level python user code to low-level c code. In this complicated system, anything could potentially become the major bottleneck, and the bottleneck contribution of each component could vary a lot under different software and hardware environments. Comprehensiveness is therefore desired from two aspects: first, the profiler should be able to reveal most approaches that are promising for speed-up; second, the profiler should avoid missing unexpected bottlenecks that might damage the performance improvement of a certain approach.

%Another requirement for profiling tools is the interpretability. A good interpretability should allow users to easily understand performance bottlenecks and quickly see the potentials of different optimization approaches. The tools we mentioned in section~\ref{motiv:limit} have shown several levels of result interpretability, ranging (low to high) from metrics numbers, a timeline view, to making predictions. Figure (TODO) shows a comparison of these profiling tools mentioned in~\ref{motiv:limit} along the dimensions of comprehensiveness and interpretability. We can see there exists a general trade-off between these two dimensions.

%To overcome the limitations of existing profiling tools and achieve both comprehensiveness and interpretability, we propose a new profiling system called \system{}. to collect the low-level details, structure them, and present directly intuitive profiling results to users. Figure (TODO) shows the overall structure of \system{}. (TODO)

%\textbf{Challenge 1: Delivering intuitive profiling results.} The requirement of performance prediction raises the problem of which are the right what-if questions for the tool to answer. A random prediction might have promising speed-up numbers, but poor feasibility for implementation. Therefore, a meaningful prediction question should connect directly to certain approach that are feasible by certain people, and meanwhile has the potential to deliver outstanding speed-up.

%\textbf{Challenge 2: Closing the gap between low-level details and high-level results.} Vendor-provided tools expose vast amount of low-level hardware counters to help profile various DNN workloads. However, these details are often hard for people to interpret. Researchers have built a few benchmarking and profiling tool chains (e.g. Fathom, TBD, MLModelScope, etc.) on top of low-level profiling tools. These tool chains collect the low-level details and extracting meaningful performance metrics out of them, bringing insights about optimization opportunities. Despite that these tool chains help improve the interpretability of profiling results, it still requires certain amount of domain expertise to identify the best improvement opportunities. We think the next generation of profiling tools should be able to reduce the expertise required and reveal the improvement opportunities by predicting performance when people use certain approaches.

In this section, we describe the challenges to build \system{}, and the key observations behind the \system{}'s design.

\subsection{Need for Kernel-level Granularity} \label{sec:motiv:kernel}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/profile_mxnet.png}
    \caption{MXNet profiler example}
    \label{fig:mxprofile}
\end{figure}

Most mainstream DNN frameworks provide built-in profiling tools to help programmers understand the "where time goes" question. Such profile is often presented in the layer-level abstraction.
Figure~\ref{fig:mxprofile} shows a fragment of the profile generated by MXNet (opened with \url{chrome://tracing}). One box in this profile represents the forward phase of one layer. It shows how much time does each layer spend in a succinct way, but does not expose details inside the runtime of a layer (e.g., how much time is spent on CPU or GPU).

When estimating performance of techniques that optimize the computation in hardware accelerators, the layer-level abstraction could be too high-level, which will likely cause huge prediction error.
One of such examples is the mixed precision~\cite{das2018mixed} technique.
If we estimate the overall performance by scaling each layer by 2x, we are very likely to predict the overall speedup to be close to 2x (and higher when considering Tensor Cores).
However, as we show later in Section~\ref{sec:eval:amp}, the speedup of mixed precision could be much lower than 2x.
Such prediction error is due to lack of low-level runtime information.
The runtime scale of any given layer depends on the concurrency between the CPU and GPU runtime, and the types of GPU kernels (compute-bound or memory-bound). 
Hence, to accurately estimate such optimizations, it is necessary to model them in the kernel-level abstraction, i.e., each GPU kernel corresponds to one individual \task{} in the dependency graph.

\subsection{Challenge 1: Constructing the Graph} \label{sec:motiv:chlg1}

\begin{figure}
    \subfloat[NVProf timeline of training ResNet-50. \label{fig:nvprof_resnet50}]{\includegraphics[width=\columnwidth]{figures/nvprof_resnet50.png}}
    \hspace{0.3cm}
    \subfloat[NVProf timeline of BERT\textsubscript{LARGE}.\label{fig:nvprof_bert_l}]{\includegraphics[width=\columnwidth]{figures/nvprof_bert_large.png}}
    \caption{NVProf timeline examples.}
    \label{fig:nvprof_screenshots}
\end{figure}

DNN training is an iterative algorithm that each iteration performs the same forward and backward computation. Predicting performance should be based on profiles from at least one iterations. A kernel-level \task{} could be less than twenty microseconds. Nevertheless, one DNN training iteration typically takes a few hundreds milliseconds. This suggests that the number of \task{}s in a graph is expected to be at least hundreds or even thousands. Manually adding dependencies for all \task{}s will be challenging as the dependency graph topology could be very complicated.

We observe a few key features of DNN training workloads that make the graph construction feasible. First, once a minibatch has been prepared by data loading threads, only one or two CPU threads are involved in the control path of computation. Second, there are also zero or very limited concurrent GPU kernels. Figure~\ref{fig:nvprof_screenshots} shows the NVProf profiles of one training iteration of the ResNet-50 and BERT\textsubscript{LARGE} models. There are two CPU threads involved, but no CPU \task{}s run concurrently. Similar to CPU and GPU \task{}s, communication \task{}s that go through the same network channel are also serialized. % hongyu: do we need to explain the communication part?

There are three main reasons that cause the \task{}s to be highly serialized: (i) the implementation of mainstream DNN frameworks rarely invoke sub-processes; (ii) the GPU kernels in modern cuDNN library achieve high GPU core utilization; (iii) some mainstream frameworks invoke only one or very few GPU streams. Due to the serialized property of massive low-level \task{}s in DNN training workloads, all \task{}s in a dependency graph can be essentially viewed as a few linked lists, and we only needs to determine the dependencies across these linked lists.

\subsection{Challenge 2: Modifying the Graph} \label{sec:motiv:chlg2}

The design of \system{} considers not only how to construct the graph (so that we can accurately simulate the execution), but also how to properly modify the graph according to common optimizations for DNN training. Describing these optimizations often requires concepts across different levels of abstractions. One of the examples is the FusedAdam optimizer provided by NVidia's Apex package. This optimizer fuses all kernels in the Adam optimizer into one single kernel. To properly change the graph, we need to know which \task{}s belong to the weight update phase. It is very onerous to manually add/delete node by node and edge by edge in a kernel-level dependency graph. To enable easy and accurate graph modification based on optimizations require: (1) mapping \task{}s to DNN layers; (2) introducing a set of graph-changing rules that are easy to use.



==> sections/scalability.tex <==

\section{Predictive Analysis} \label{sec:predict}

%The most commonly used scheme for distributed deep learning training is data parallelism. This type of parallelism assigns a model replica and a subset of data samples to each worker. The minibatch size will also increase proportionally with the number of GPUs so that the computation power of a single GPU is still fully exploited. This will affect two things: the model convergence, and the scalability. Both of them will affect the end-to-end training time.

%Researchers have proposed several rules to ensure that the convergence of training on large minibatch size is as good as training on small minibatch size (TODO cite). On the performance side, using distributed training will introduce communication overhead as one of the major bottlenecks. Besides spending money for higher bandwidth networks, researchers tried various approaches to reduce communication overhead, and make DNN training scalable under low-bandwidth commodity network. These approaches can be categorized into two major types:

%\begin{itemize}
%    \item \textbf{Reducing Communication Time}. Examples are gradient compression, quantization, PASGD, etc. (TODO: cite a lot)
%    \item \textbf{Overlap Communication wigh Computation}. Examples are asynchronous SGD, wait-free weight reduction, TicTac, P3, etc. (TODO: cite a lot)
%\end{itemize}

In this section, we evaluate NeuralTap's prediction accuracy for distributed training under different system configurations, and also explain why the performance predictions are inaccurate for Deep Speech 2.

%\subsection{How do We Predict Scalability and Improvements of Optimizations?}

%As described in section~\ref{sec:impl}, NeuralTap relies on a dependency graph approach to accurately predict the performance for distributed training. This approach first breaks down the per-iteration training process into small tasks, and determine the execution dependencies among them. We then estimate the running time of each task either by measuring or predicting, and simulate the execution to determine the total running time. We find that the followings are crucial for making accurate predictions using this approach:

%\begin{itemize}
%    \item \textbf{Job Breakdown.} Beyond layer-wise communication and computation, the training process will have other workloads, which could become bottleneck unexpectedly under different models or hardware environments. A good example is weight update. As we can see from section~\ref{sec:util}, it could be a major bottleneck for BERT, but a minor bottleneck for seq2seq and ResNet-50.
%    \item \textbf{Task Granularity.} As desbribed in section~\ref{sec:impl:gran}, task granularity plays a key role in making accurate predictions. A granularity that is no matter too small or too large will negatively affect the prediction accuracy.
%    \item \textbf{Scheduling of Communications.} The scheduling of communications will affect how the communication tasks are simulated. This is determined by the execution dependencies among the tasks, which could be caused by data dependencies, or synchronization inherent inside the implementation.
%    \item \textbf{Size of Gradients.} According to the model, the size of gradients to be transferred can vary a lot. This will determine the running time of each individual communication task.
%    \item \textbf{Hardware Environments.} The network or PCIe bandwidth will greatly affect the running time of each communication. The computation running time will also changes on different GPUs.
%    \item \textbf{Software Environments.} The bandend implementation of communication primitives will also affect the communication time and dependencies. Our following evaluations will base on NCCL backend, as it works better than other options in PyTorch for our testing workloads. NCCL provides fast communication primitives, however it doesn't allow two communication primitives running concurrently.
%\end{itemize}

%Considering the low-level profiling tools that are available for us to use, NeuralTap breaks down the training process into following types of tasks: data loading, layer-wise computation, weight update, and communication. A computation task is either the forward or a backward of certain layer defined by PyTorch APIs. A communication task is an individual NCCL reduction.

%The breakdown of training process and dependencies among tasks can be determined in a single-GPU environment, without actually running on a distributed environment. The running time of data loading, layer-wise computation and communication can also be measured in a single-GPU environment if the required type of GPU is available (Figure~\ref{fig:mapping}). The running time of NCCL primitives, on the other hand, is impossible to measure but can only be estimated without a distributed environment.

\subsection{Predicting Scalability}

\begin{figure}
    \centering
    \subfloat[Runtime predictions for ResNet-50.\label{fig:sync_reduce_resnet}]{\includegraphics[width=\columnwidth]{figures/prediction_error_resnet.pdf}}
    
    \subfloat[Runtime predictions for Seq2Seq.\label{fig:sync_reduce_resnet}]{\includegraphics[width=\columnwidth]{figures/prediction_error_seq2seq.pdf}}
    
    \subfloat[Runtime predictions for Deep Speech 2.\label{fig:sync_reduce_ds2}]{\includegraphics[width=\columnwidth]{figures/prediction_error_ds2_new.pdf}}
    
    \subfloat[Runtime predictions for BERT\textsubscript{BASE}.\label{fig:sync_reduce_bert_base}]{\includegraphics[width=\columnwidth]{figures/prediction_error_bert_base.pdf}}
    
    \subfloat[Runtime predictions for BERT\textsubscript{LARGE}.\label{fig:sync_reduce_bert_large}]{\includegraphics[width=\columnwidth]{figures/prediction_error_bert_large.pdf}}
    \caption{The error between NeuralTap's runtime predictions and the baseline with synchronization before each allReduce under various system configurations.}
    \label{fig:predict_scalalibity}
\end{figure}

Figure~\ref{fig:predict_scalalibity} shows the comparisons between runtimes predicted by NeuralTap and the ground truth runtimes measured for each DNN model under different system configurations. We evaluate the prediction accuracy for both PCIe connected multi-GPU systems and Ethernet/InfiniBand connected multi-machine systems under different network bandwidths (10, 20, 40 Gbps). Except for the Deep Speech 2 model, NeuralTap achieves prediction error of less than 10\% for all configurations, and around or even less than 5\% for most configurations.
For the Deep Speech 2 model, we observe that the prediction error is generally higher than 10\%, and positively correlated with the number of GPUs. Compared to the two-GPU configuration, the prediction error of 8 GPUs is 10\% to 15\% higher.

%For the Deep Speech 2 model, the prediction error is generally higher than 10\%. With bandwidth of 10Gbps, the error is between 10\% and 20\%. The error increases to between 14\% and 36\% under 40Gbps bandwidth. This is because the prediction error for communication increases as the bandwidth is higher (as we show in Figure~\ref{fig:prediction_error_bw}). The prediction error is also largely affected by the number of GPUs. Compared to the two-GPU configuration, the prediction error of 8 GPUs is 10\% to 16\% higher depending on the bandwidth. We conclude that for Deep Speech 2 model, the prediction error is positively correlated with the bandwidth and the number of GPUs.

\subsection{Why Prediction Errors are High for Deep Speech 2?}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/time_mem.pdf}
    \caption{The iteration time of GPU 0, and memory footprint of two GPUs when using two GPUs to train Deep Speech 2.}
    \label{fig:time_mem}
\end{figure}

There are several reasons why the predictions are inaccurate for Deep Speech 2, and most of them are application-specific. We found that the major cause for the prediction error is the memory management policy and batching strategy as mentioned in Section~\ref{sec:util:ds2}. Figure~\ref{fig:time_mem} shows the iteration time for the first two hundreds iterations of training Deep Speech 2 using two GPUs, along with the memory footprint of each GPU. We observe that there are outlier iterations when a GPU releases all the memory allocated dynamically from previous training iterations.

To handle the variable length of data samples in the LibriSpeech dataset, the training process will first sort all data samples by length before forming mini-batches for different GPUs. This batching strategy minimizes the padding added to short data samples, but also makes the dynamic memory among different GPUs accumulate at different paces. Therefore, different GPUs likely release their memory at the different iteration. Every time the memory consumption of a GPU hits the GPU memory capacity (11GB in this experiment), all other GPUs have to wait for it to release its memory. In Figure~\ref{fig:time_mem}, the iteration time spikes when either GPU 0 or GPU 1 releases their memory. This overhead will increase as we scale up, causing higher prediction error when training Deep Speech 2 with more GPUs.

%Such outliers are rare on other DNN applications, as most DNN applications allocate memory statically before training iterations start. Predicting runtime caused by this overhead requires monitoring memory usage and measuring the memory management cost. Meanwhile, the prediction error caused by increasing network bandwidth suggests that communication is another cause for prediction error, which can be potentially mitigated by considering detailed runtime statistics of concurrent GPU kernels. Both fixes are orthogonal to current NeuralTap design, and does not change the mechanism of NeuralTap profiling workflow.

Such outliers are rare on other DNN applications, as most DNN applications allocate memory statically before training iteration starts. Capturing this overhead in our runtime prediction model requires monitoring memory usage and measuring the memory management cost, which is orthogonal to current NeuralTap design, and does not fundamentally change the NeuralTap profiling workflow.


==> sections/sketch.tex <==
\section{Sketch}

This section will be removed.

\begin{comment}
\subsection{Hightlights in section 2 (Motivations and Goals)}

Motivations:
\begin{itemize}
    \item \textbf{Motivation 1}: Low interpretability. Hardware profiling tools provide comprehensive hardware counters, but requires extra efforts, and experiences on system and hardware to interpret and assemble the results. (M1)
    \item \textbf{Motivation 2}: Current approach of measuring layer span using synchronization (used by existing framework built-in tools) is intrusive. This could lead to overlooked bottlenecks and opportunities. (M2)
    \item \textbf{Motivation 3}: Optimizations using multiple GPUs or multiple machines are often consuming in time (for software) or money (for hardware). It is therefore desired to predict the performance to help decide the most promising approach, before spending time or money. (M3)
\end{itemize}

Goals of NeuralTap:

\begin{itemize}
    \item \textbf{Goal 1}. Enable suggesting the most promising way to speed up training, by predicting performance and identify bottlenecks. (G1, --> M2, M3)
    \item \textbf{Goal 2}. Help programmers correlate low-level inefficiency to high-level code. (G2, --> M1)
\end{itemize}
\end{comment}

\subsection{Backgrounds (before Motivation)}

\begin{itemize}
    \item Summary of existing optimization strategies for DNN training
    \item Summary of existing profiling tools (hardware profiling tools, framework built-in tools, performance oracles)
    \item Previous similar works on other fields (e.g. for Sparks), introduce the dependency graph analysis
\end{itemize}

\subsection{Hightlights in section 3 (Requirements and Designs)}
\subsubsection{Requirements}

\begin{itemize}
    \item \textbf{Requirement 1}: The profiling tool should present profiling results based on potential performance optimization strategies.
    \item \textbf{Requirement 2}: Performance prediction should achieve high accuracy at low costs.
    \item \textbf{Requirement 3}: The profiling tool should also be aware of optimization opportunities in the single-GPU environment, as well as multi-GPU and multi-node environments.
\end{itemize}

\subsubsection{Bottlenecks in Single-GPU Environments}

(Move section 5.1 here) Introduce the breakdown of CPU-only, GPU-only, CPU+GPU parallel runtime.

\subsubsection{Overview of NeuralTap}

Design flow focuses on how to organize the data collected by hardware profiling tool:

Design flow of bottleneck profiling:

\begin{itemize}
    \item \textbf{Step 1} Using nvprof/cupti/timing to extract low-level runtime information based on execution on a single GPU environment.
    \item \textbf{Step 2} Map CPU APIs and GPU kernels to layers.
    \item \textbf{Step 3} Analyze the CPU-GPU runtime breakdown.
    \item \textbf{Step 4} ...
\end{itemize}

Design flow of predicting performance:

\begin{itemize}
    \item \textbf{Step 1} Using nvprof/cupti/timing to extract low-level runtime information based on execution on a single GPU environment.
    \item \textbf{Step 2} Predict reduction time based on data size and bandwidth
    \item \textbf{Step 3} Simulate runtime
    \item \textbf{Step 4} ...
\end{itemize}

\subsubsection{Timing accelerators without additional synchronizations}

\begin{itemize}
    \item Show how synchronization lead to different runtime. (Move section 5.2 kernel-waiting operations here)
    \item Show how to implement synchronization-free kernel-to-layer Mapping.
\end{itemize}

\subsubsection{Predicting}

\begin{itemize}
    \item Reduction time needs to be calculated accurately, to achieve high prediction accuracy at low cost
    \item Show how other GPU kernels affect reductions (adding synchronizations before and after reduction)
    \item Show how to calculate on reduction time on n GPUs (things are different for multi-node and multi-GPU)
\end{itemize}

==> sections/utilization.tex <==

\section{Bottleneck Analysis} \label{sec:util}

In this section, we discuss how NeuralTap can identify performance bottlenecks and provide programmers hints about optimizations that improve hardware utilization. In the particular cases of Deep Speech 2 and BERT, we show how NeuralTap helps identify the root causes for the CPU bottlenecks.
%This bottleneck analysis reveals optimization opportunities that lead to 15\% speedup, with less than 30 lines of code changes in total.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/breakdown_all.pdf}
    \caption{The CPU-GPU runtime breakdown of all models. The GPU compute utilization is the sum of GPU-only and CPU+GPU runtime.}
    \label{fig:breakdown_all}
\end{figure}

Figure~\ref{fig:breakdown_all} shows a high-level CPU-GPU runtime breakdown for each model. Both ResNet-50 and Seq2Seq models achieve high GPU compute utilization (over 90\%). The large portion of GPU-only runtime in ResNet-50 and Seq2Seq suggests that GPU computation is the main bottleneck, and therefore reducing GPU runtime (e.g, by reducing precision~\cite{das2018mixed}~\cite{gupta2015deep}~\cite{micikevicius2017mixed}) will potentially be an effective optimization strategy. This strategy could also be effective for BERT\textsubscript{BASE}, but not for BERT\textsubscript{LARGE} since its GPU-only runtime is only 14\% of the total runtime. In the rest of this section, we will use the training of BERT and Deep Speech 2 models as examples, to show how the NeuralTap profiling workflow (Section~\ref{sec:idea:overview}) helps pinpoint the bottlenecks, and further identify optimization opportunities when GPU computation is not the major bottleneck.

\subsection{Use Case \#1: Training BERT} \label{sec:util:bert}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/breakdown_cpu.pdf}
    \caption{The layer-wise breakdown of CPU-only runtime of BERT and Deep Speech 2. The Forward/Backward Gaps parts denote the runtimes of gaps among forward/backward layers.}
    \label{fig:breakdown_cpu}
\end{figure}

\begin{figure}
    \centering
    \subfloat[The CPU-only runtime breakdown in weight update of training BERT.\label{fig:breakdown_adam}]{\includegraphics[width=0.48\columnwidth]{figures/breakdown_adam.pdf}}
    \hspace{0.2cm}
    \subfloat[The CPU-only runtime breakdown in gaps among forward layers of training Deep Speech 2.\label{fig:breakdown_ffgaps}]{\includegraphics[width=0.48\columnwidth]{figures/breakdown_ffgaps.pdf}}
    \caption{The CPU-only runtime breakdown according to CUDA APIs. For BERT we show the breakdown for the weight update phase, for Deep Speech 2 we show the breakdown for the intervals between consecutive layers in the forward phase.}
    \label{fig:breakdown_hotspots}
\end{figure}

As we show in Figure~\ref{fig:breakdown_all}, the GPU is idle for 20.2\% and 35.2\% of the total runtime for BERT\textsubscript{BASE} and BERT\textsubscript{LARGE} models respectively. For BERT\textsubscript{LARGE}, the GPU-only runtime accounts for only 14.1\% of the total runtime, suggesting that the CPU runtime is a major bottleneck. 
%NeuralTap analyzes the cause of the CPU-only bottleneck by fine-grained breakdown at the granularity of DNN layers and CUDA APIs respectively. 
Figure~\ref{fig:breakdown_cpu} shows the fine-grained breakdown of the CPU-only runtime according to training phases. The Forward/Backward Gaps in Figure~\ref{fig:breakdown_cpu} denote the duration between consecutive layers in the forward/backward phase. Based on the breakdown results, we make the following observation:

\textbf{Observation 1: The majority of the CPU-only runtime is contributed by the weight update phase.} Figure~\ref{fig:breakdown_cpu} shows the layer-wise breakdown of the CPU-only runtime in one iteration. For the training of BERT\textsubscript{BASE}, 87.6\% of the CPU-only runtime comes from the weight update phase, which is 17.5\% (20.2\% times 87.6\%) of the total runtime. For the training of BERT\textsubscript{LARGE}, 58.5\% of the CPU-only runtime comes from the weight update phase, which is 20.6\% (35.2\% times 58.5\%) of the total runtime.

Figure~\ref{fig:breakdown_adam} shows the fine-grained breakdown of the CPU-only runtime during the weight update phase of training BERT models with respect to CUDA APIs. The breakdown results suggest the following observation:

\textbf{Observation 2: During the weight update phase, the CPU-only runtime is mainly caused by launching kernels.}  Figure~\ref{fig:breakdown_adam} shows that the CPU-only runtime is contributed by mainly three parts: (i) \texttt{cudaLaunchKernel}, (ii) \texttt{cudaGetDevice}, and (iii) non-CUDA C/Python functions. A \texttt{cudaLaunchKernel} API is implicitly invoked when the CPU program launches a kernel onto the GPU and incurs non-negligible overhead. In modern DNN frameworks, launching a CUDA kernel is a deep call stack from user program to low-level CUDA program, which involves overhead from non-CUDA functions and potentially other CUDA APIs (e.g. \texttt{cudaSetupArgument}, \texttt{cudaConfigureCall}). We also observe that PyTorch invokes a substantial number of \texttt{cudaGetDevice} APIs when launching kernels.

%These two observations are derived from the NeuralTap profiling results of breaking down the CPU runtime according to layers or CUDA APIs, without extra programmer effort (described in Section~\ref{sec:motiv}). 
Based on these observations, we conclude that the major cause for the CPU bottleneck is launching numerous small kernels in the weight update phase, which can be effectively optimized by the kernel fusion technique~\cite{ashari2015optimizing}.
How to implement kernel fusion efficiently, however, is usually application-specific. Our implementation of the optimization adopts concatenation of the gradients, so that in each weight update phase, element-wise kernels for different layers are fused into a single GPU kernel. This optimization greatly reduces the overhead of launching numerous small kernels. As a result, we achieve 10\% and 14\% speedups for training BERT\textsubscript{BASE} and BERT\textsubscript{LARGE} respectively, with only up to 20 lines of code change in total.

%\textbf{Observation 2: Almost all of the GPU-only runtime is concentrated in the end of backward pass.} Figure~\ref{fig:bert_timeline} shows the visualized CPU and GPU runtimes of one iteration in timeline view. This timeline shows that the GPU-only runtime is 

%The second observation suggests that we can potentially overlap the CPU-only runtime in updating weights with the GPU-only runtime in backward pass, by removing synchronizations in the backward pass. However, simply removing the \texttt{cudaStreamSynchronize} does not improve the overall performance. This is because there are \texttt{cudaMemcpyAsync} calls that will also force the CPU to wait for the backward pass to complete. With the help of the layer mapping feature of NeuralTap, we manage to locate that synchronizations and memory copies that need to be removed come from three different code locations in framework:

%\begin{itemize}
%    \item \textbf{Location 1: the \texttt{sort\_by\_key} function of thrust library in the backward of embedding layer}. This function implicitly calls \texttt{cudaStreamSynchronize} before calling its own sorting kernels. We replace it with a new implementation that has no synchronization involved.
%    \item \textbf{Location 2: calculating norm of tensors when clipping the gradients}. The low-level implementation of norm calculation puts result on CPU, and then copy the results back to GPU if the input is on GPU. This will implicitly invoke \texttt{cudaMemcpyAsync} which waits on CPU until the result being calculated. We replace it by using summation and power operations, shown by the following formula:
%        \begin{equation}
%        norm(p)=power(sum(power(p,2)),0.5)
%        \label{for:reduce_p2p}
%        \end{equation}
%    \item \textbf{Location 3: comparing the norm with a threshold when clipping the gradients}. This simple if statement in PyTorch will implicitly invoke \texttt{cudaMemcpyAsync}. We replace this by clamping the norm with threshold before the element-wise multiplication.
%\end{itemize}

%Figure~\ref{fig:bert_opt_timeline} shows the timeline after we apply the implementation changes described above. Ideally, a perfect overlap will hide all of the CPU-only runtime in weight updates, which brings roughly 16\% (19.7\%x81.2\%) speedup. However, it turns out that the changes we made achieve only 5\% speedup. This is due to the limitations of current PyTorch user APIs. The changes in location 2 and 3 involve using extra for each layer.

\subsection{Use Case \#2: Training Deep Speech 2} \label{sec:util:ds2}

Similar to BERT\textsubscript{LARGE}, the CPU runtime is a major bottleneck for training Deep Speech 2 (as we show in Figure~\ref{fig:breakdown_all}). However, in contrast to BERT\textsubscript{LARGE}, 50.1\% of the CPU-only runtime is consumed by the gaps among forward layers (as we show in Figure~\ref{fig:breakdown_cpu}), where no GPU kernels are invoked typically.
%This suggests that the cause to the CPU bottleneck in training Deep Speech 2 is different from that of the BERT models (launching numerous small kernels).

Figure~\ref{fig:breakdown_ffgaps} shows the fine-grained breakdown of the runtime gaps between layers in the forward phase of training Deep Speech 2. The CUDA launch part is almost negligible (only 3.1\%), instead there is a large portion of time spent on C/Python functions and \texttt{cudaFree} calls. The \texttt{cudaFree} calls suggest that memory management could be a major cause for the CPU bottleneck. By examining the baseline implementation of the forward phase, we observe that the main overhead of CPU runtime is caused by memory allocations and data initializations. These allocations are executed in every iteration, causing accumulation of the memory footprint during training iterations, as well as periodic memory deallocations to avoid memory overflow.

The main reason why memory is managed dynamically for Deep Speech 2 is due to its batching strategy. The speech recognition task uses data samples of variable lengths\footnote{In the LibriSpeech dataset, the lengths of audio files range from one or two seconds to tens of seconds~\cite{panayotov2015librispeech}}. When forming a mini-batch, short data samples will be padded to have the same length as the longest sample in the same mini-batch. Therefore, the length of the mini-batch, as well as the size of most intermediate results, will vary over iterations. The overhead of dynamic memory management can be potentially reduced by using a fixed length for all mini-batches, but extra padding will also waste compute resources.

Based on our insights about the cause of CPU bottlenecks, we implement an optimization which allocates and initializes intermediate data on GPU directly, avoiding the overhead of data initialization on CPU and data transfer from CPU to GPU. We also utilize the idea of kernel fusion from optimizing BERT training (Section~\ref{sec:util:bert}) to optimize the weight update phase of Deep Speech 2 by concatenating the gradients. We ultimately manage to improve the training performance of Deep Speech 2 by 15\%. Our implementation involves changes in three locations from the baseline code, with less than 10 lines of code changes for each location.

%Figure~\ref{fig:ds2_breakdown} shows the layer-wise breakdown of the CPU-only runtime. As we can see, the majority (60\%) of CPU-only runtime resides in the gaps between the forward pass, while the rest is scattered across various parts in runtime. This is good news for performance profiling, because in PyTorch the computation of the forward pass is directly defined by python programs, so there is more chance to fix loopholes by only local changes. If we further breakdown the CPU-only runtime in forward pass, we observe big gaps among the convolutional layers. This helps us locate a loophole in the implementation of the convolutional layers, which can be fixed with 10 lines of local code change.

%Another loophole we located in the gaps between forward layers is data locality. The data batch size in Deep Speech 2 has variable lengths, therefore the dimensions of inputs and outputs tensors have to be computed during training. These tensors need to be used for the computations of all layers in the RNN stack, which is the main body of the Deep Speech 2 model. If these dimension tensors are not properly placed on GPU, redundant memory copies will be implicitly invoked. We fix this loophole by changing only 2 lines in the source code.

%Besides the runtime in the gaps of forward layers, the rests of CPU-only runtime reside in mainly three places: the gaps between the backward layers, the computations of the backward layers, and the weight update of SGD optimizer. We didn't find easy local changes that can cut the CPU-only runtime in either the backward layers themselves or the gaps of these layers. This is because the backward runtime of PyTorch is defined in its autograd engine which is implemented in C backend. Cutting the CPU-only runtime in the backward process requires changes in the forward pass, or inside the C code base.

%In the runtime of weight update, we found that cudaLaunch contributes a major part of the CPU-only runtime. This is due to the inefficient implementation of the clip\_norm operation. In PyTorch, the default implementation of the clip\_norm operation calls norm computation for each single gradient tensors, resulting in many tiny GPU kernels and their cudaLaunch functions becoming the bottleneck. We optimize the implementation by merging small gradient tensors of a layer into a single tensor and calculating the norm only once for a layer. Combining all the optimizations, we manage to reduce the CPU-only runtime from 39\% to 19\% with less than 20 lines of code changes, achieving around 15\% speed up on average.

%\subsection{How to Predict Performance if Certain Kernels Utilize GPU More Efficiently?}

%GPU is a many-core architecture, how efficient a GPU kernel utilize its ALU cores is crucial for the performance of that GPU kernel. The most direct way to improve the core utilization of GPU kernels is to increase minibatch size. Within the memory budget, machine learning people usually increase the minibatch size to the greatest extent. To further increase the minibatch size requires techniques to reduce the memory footprints. As the minibatch size increases, the training throughput will eventually saturate. In this case, we have to consider improving the implementations of GPU kernels with low core utilization if we want to reduce GPU runtime.

%The most straight-forward approach to predict kernel performance, either with a new implementation or under different minibatch size, is to model the execution time of that kernel. This approach is not scalable because we have to potentially model for each individual kernel. A more fundamental approach is to understand the GPU architecture and simulate kernel executions. For a close-sourced library like cudnn, this is very hard because the underlying implementation is not revealed for simulation, and the same kernel might behave differently when GPU or any function parameter changes. Beyond predicting execution time of individual kernels, the profiler has to consider CPU-GPU overlap to predict total execution time, only speeding up kernels in critical path can speed up the total execution time. This is overall a complicated problem for future works.

